Empirical Privacy Variance

We propose the notion of empirical privacy variance and study it in the context of differentially private fine-tuning of language models. Specifically, we show that models calibrated to the same $(\varepsilon, \delta)$-DP guarantee using DP-SGD with different hyperparameter configurations can exhibit significant variations in empirical privacy, which we quantify through the lens of memorization. We investigate the generality of this phenomenon across multiple dimensions and discuss why it is surprising and relevant. Through regression analysis, we examine how individual and composite hyperparameters influence empirical privacy. The results reveal a no-free-lunch trade-off: existing practices of hyperparameter tuning in DP-SGD, which focus on optimizing utility under a fixed privacy budget, often come at the expense of empirical privacy. To address this, we propose refined heuristics for hyperparameter selection that explicitly account for empirical privacy, showing that they are both precise and practically useful. Finally, we take preliminary steps to understand empirical privacy variance. We propose two hypotheses, identify limitations in existing techniques like privacy auditing, and outline open questions for future research.

==> 1_intro_chiyuan.tex <==
\section{Introduction} \label{sec:intro}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{fig/fig-overview.pdf}
    \caption{Caption}
    \label{fig:overview}
\end{figure}

Modern large language models (LLMs) exhibit remarkable proficiency in a multitude of domains, from traditional natural language processing problems such as summarization and translation, to complex problem solving that involves reasoning, planning, mathematics and coding. Those models are trained on massive datasets with more than $10^{13}$ tokens~\citep{dubey2024llama,team2024gemma}, collected from various sources such as Wikipedia, open source code repositories, public domain books, and public forums. While most of data comes from the public web, they could still contain sensitive personal information accidentally leaked over the Internet, and the scale of the data makes it extremely challenging to completely filter out sensitive information. Moreover, due to the increasingly popular application of LLMs as chatbots or even personalize agents, there is growing interest in the possibility of training with user data to adapt to real world usage cases and human preferences. The pressing concern of user privacy has fueled a proliferation of research on training LLMs with differential privacy~\citep[DP,][]{dwork2014algorithmic} protection~\citep{anil2021large,yu2022differentially,he2022exploring,li2022large,bu2023differentially,wu2024privately}. 
\fan{last part duplicated with content in preliminaries}

However, while DP is a widely accepted notion of privacy with formal gurantees, the numerical values of the privacy parameters are not very easily interpretable. Specifically, in real world interactions with LLMs, a common privacy concern is having the model generate text containing sensitive information (e.g. some people's credit card number) it has seen during training. Numerous studies have demonstrated that this kind of memorization and regurgitation is a real challenge of privacy that needs to be addressed LLM applications~\citep{carlini2021extracting,carlini22quantifying,lukas2023analyzing,biderman2024emergent,prashanth2024recite}. While DP training generally helps, it is unclear how to relate the privacy bounds of DP to the empirical privacy measures that quantifies the amount of memorization in LLMs. In this paper, we provide the first systematic study to link the two measures, and uncover an important phenomenon of \emph{empirical privacy variance}: LLMs calibrated to the same (quantitative) DP guarantee can exhibit significant variations in empirical privacy measures. We summarize our main contributions in the following:

We demonstrate the \emph{empirical privacy variance} phenomenon in \Cref{sec:variance}, and verify its generality across multiple datasets and empirical privacy measures. In \Cref{sec:hyperparameter} we conduct in-depth analysis of how common hyperparameters influence the empirical privacy and provide recommendations for hyperparameter selections. Our analysis reveals important trade-off between formal DP guarantee and empirical privacy measure, allows practitioners to make proper hyperparameter choices depending on their specific privacy requirements. Finally, in \Cref{sec:understanding}, we explore a number of hypothesis in order to demystify this phenomenon and identify important open questions along this direction.

\fan{
other motivation to involve in the intro:

\textbf{people's understanding/expectation for DP}

\citet{nanayakkara2023chances}: ``people struggle to reason
about probabilistic risks.''

\citet{cummings2021need}: ``the ways in which differential privacy is described in-the-wild
haphazardly set users’ privacy expectations, which can be misleading''

\citet{xiong2020towards}
``When shown descriptions that explain the implications instead
of the definition/processes of DP or LDP technique, participants
demonstrated better comprehension and showed more willingness
to share information''

$\rightarrow$ what's the implication of DP on \empv? can we expect consistency?
}



==> 1_intro_new.tex <==
Modern large language models (LLMs) demonstrate remarkable proficiency across a wide range of domains, including summarization, translation, and complex problem-solving tasks such as reasoning and coding~\citep{stiennon2020learning,barrault2023seamless,huang2023towards,roziere2023code}. 
These capabilities are powered by pre-training on massive datasets~\citep{dubey2024llama,team2024gemma}.
To meet real-world needs, a growing paradigm involves fine-tuning pre-trained models on downstream tasks or user-specific data, enhancing domain applicability and personalization~\citep{guo2022domain,li2024personal}.
However, this process introduces significant privacy concerns, as fine-tuning datasets often contain sensitive information of individuals or organizations. 
Compounding these concerns, LLMs have demonstrated a strong capacity to memorize their training data~\citep{carlini2021extracting,carlini22quantifying,lukas2023analyzing,biderman2024emergent,prashanth2024recite}.

In response, differential privacy (DP)~\citep{dwork2014algorithmic}, the gold standard for privacy protection, has been incorporated into various stages of LM fine-tuning. This has driven a fruitful line of research advancing the utility-privacy trade-off in LLMs~\citep{anil2021large,yu2022differentially,li2022large,bu2023differentially,wu2024privately}.
Nevertheless, privacy in language models is a nuanced and multifaceted concept. The complexities arise not only from the nature of private information in natural language, which is often unstructured and context-dependent~\citep{brown2022does}, but also from the generative nature of LLMs. Unlike discriminative models, generative LLMs directly produce text, creating a more immediate and tangible perception of privacy leakage during user interactions~\citep{sebastian2023privacy,falcao2024investigating}.
This introduces a practical perspective on privacy that centers on human perceptions of model behaviors like memorization and regurgitation, an aspect we broadly term \textit{empirical privacy}. Therefore, when applying DP to LLMs, there is a mismatch  between the theoretical guarantees that DP offers and the empirical privacy that people care about in the real world. In fact, this disconnect has long been a challenge in conveying the prospect of DP to broader audiences~\citep{nanayakkara2023chances,cummings2021need}, as research shows that people better understand implications rather than formal definitions~\citep{xiong2020towards}.
Thus, the key question emerges: \textit{What are the implications of DP for empirical privacy in LLMs?}

==> _1-summary.tex <==
This work uncovers a phenomenon termed \textit{empirical privacy variance} in the differentially private fine-tuning of language models. Specially, we
show that models calibrated to the same $(\varepsilon, \delta)$-DP guarantee using DP-SGD with different hyperparameter configurations can exhibit significant variations in empirical privacy, which we quantitatively measure through the lens of memorization. 
We investigate the generality of this phenomenon across multiple dimensions and discuss why it is surprising and practically relevant. Through regression analysis, we examine how individual and composite hyperparameters influence empirical privacy. The results reveal a no-free-lunch: existing practices of hyperparameter tuning in DP-SGD, which focus on optimizing utility under a fixed privacy budget, often come at the expense of empirical privacy. To address this, we propose guidelines for hyperparameter selection that explicitly account for empirical privacy and demonstrate their precision and practical effectiveness.
Finally, we take initial steps to demystify empirical privacy variance by proposing plausible hypotheses, identifying limitations in existing techniques like privacy auditing, and outlining open questions for future research.



==> fig_desc/fig_individual_hparam_cmp_gpt2-large_bs.tex <==
\begin{figure}


% \captionsetup[subfigure]{labelformat=empty}

\newlength{\utilheightindhparamgptlargebs}
\settoheight{\utilheightindhparamgptlargebs}{\includegraphics[width=.3\columnwidth]{fig/gpt2-large_n-13_eps-1_b-2048_lr-1e-3.pdf}}%


\newcommand{\rowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\utilheightindhparamgptlargebs][c]{\tiny #1}}}

\centering



{
\renewcommand{\tabcolsep}{10pt}



\begin{subfigure}[]{\columnwidth}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}c@{}}
        &  \makecell{\tiny{\textbf{}}}
        & \makecell{\tiny{\textbf{}}}
        &  \makecell{\tiny{\textbf{}}}
        % & \makecell{\tiny{\textbf{$p=1.0$, varying $T$}}}
        \\
&
\includegraphics[height=1.\utilheightindhparamgptlargebs]{fig/gpt2-large_n-13_eps-1_T-250_lr-1e-3.pdf}&
\includegraphics[height=1.\utilheightindhparamgptlargebs]{fig/gpt2-large_n-13_eps-2_T-250_lr-1e-3.pdf}&
\includegraphics[height=1.\utilheightindhparamgptlargebs]{fig/gpt2-large_n-13_eps-4_T-250_lr-1e-3.pdf}&
\includegraphics[height=1.\utilheightindhparamgptlargebs]{fig/gpt2-large_n-13_eps-8_T-250_lr-1e-3.pdf}&
\\[-2mm]
&
\includegraphics[height=1.\utilheightindhparamgptlargebs]{fig/gpt2-large_n-13_eps-1_T-500_lr-1e-3.pdf}&
\includegraphics[height=1.\utilheightindhparamgptlargebs]{fig/gpt2-large_n-13_eps-2_T-500_lr-1e-3.pdf}&
\includegraphics[height=1.\utilheightindhparamgptlargebs]{fig/gpt2-large_n-13_eps-4_T-500_lr-1e-3.pdf}&
\includegraphics[height=1.\utilheightindhparamgptlargebs]{fig/gpt2-large_n-13_eps-8_T-500_lr-1e-3.pdf}&
\\[-2mm]
\end{tabular}
}
\end{subfigure}
}
% \vspace{-2mm}
\caption{GPT2-large, varying batch size}%
\label{fig:ind-hparam-gpt2-large-bs}
% \vspace{-1.2em}
\end{figure}



==> fig_desc/fig_individual_hparam_cmp_gpt2-large_compute.tex <==
\begin{figure}


% \captionsetup[subfigure]{labelformat=empty}

\newlength{\utilheightindhparamgptlargecompute}
\settoheight{\utilheightindhparamgptlargecompute}{\includegraphics[width=.22\columnwidth]{fig/gpt2-large_n-13_eps-1_b-2048_lr-1e-3.pdf}}%

\newlength{\legendheightindhparamgptlargecompute}
\setlength{\legendheightindhparamgptlargecompute}{0.45\utilheightindhparamgptlargecompute}%




\newcommand{\rowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\utilheightindhparamgptlargecompute][c]{\tiny #1}}}

\centering



{
\renewcommand{\tabcolsep}{10pt}


\begin{subfigure}[]{\columnwidth}
\centering
\begin{tabular}{l}
\includegraphics[height=\legendheightindhparamgptlargecompute]{fig/legend_fix_compute_gpt2-large_cropped.pdf}
\end{tabular}
\end{subfigure}
\vspace{-1.5em}

\begin{subfigure}[]{\columnwidth}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}c@{}}
        &  \makecell{\tiny{\textbf{}}}
        & \makecell{\tiny{\textbf{}}}
        &  \makecell{\tiny{\textbf{}}}
        % & \makecell{\tiny{\textbf{$p=1.0$, varying $T$}}}
        \\
& 
\scriptsize{$\varepsilon=1$} &
\scriptsize{$\varepsilon=2$} &
\scriptsize{$\varepsilon=4$} &
\scriptsize{$\varepsilon=8$} &
\\
&
\includegraphics[height=1.\utilheightindhparamgptlargecompute]{fig/gpt2-large_n-13_eps-1_compute-512k_lr-1e-3.pdf}&
\includegraphics[height=1.\utilheightindhparamgptlargecompute]{fig/gpt2-large_n-13_eps-2_compute-512k_lr-1e-3.pdf}&
\includegraphics[height=1.\utilheightindhparamgptlargecompute]{fig/gpt2-large_n-13_eps-4_compute-512k_lr-1e-3.pdf}&
\includegraphics[height=1.\utilheightindhparamgptlargecompute]{fig/gpt2-large_n-13_eps-8_compute-512k_lr-1e-3.pdf}&
\\[-2mm]
&
\includegraphics[height=1.\utilheightindhparamgptlargecompute]{fig/gpt2-large_n-13_eps-1_compute-1024k_lr-1e-3.pdf}&
\includegraphics[height=1.\utilheightindhparamgptlargecompute]{fig/gpt2-large_n-13_eps-2_compute-1024k_lr-1e-3.pdf}&
\includegraphics[height=1.\utilheightindhparamgptlargecompute]{fig/gpt2-large_n-13_eps-4_compute-1024k_lr-1e-3.pdf}&
\includegraphics[height=1.\utilheightindhparamgptlargecompute]{fig/gpt2-large_n-13_eps-8_compute-1024k_lr-1e-3.pdf}&
\\[-2mm]
&
\includegraphics[height=1.\utilheightindhparamgptlargecompute]{fig/gpt2-large_n-13_eps-1_compute-2048k_lr-1e-3.pdf}&
\includegraphics[height=1.\utilheightindhparamgptlargecompute]{fig/gpt2-large_n-13_eps-2_compute-2048k_lr-1e-3.pdf}&
\includegraphics[height=1.\utilheightindhparamgptlargecompute]{fig/gpt2-large_n-13_eps-4_compute-2048k_lr-1e-3.pdf}&
\includegraphics[height=1.\utilheightindhparamgptlargecompute]{fig/gpt2-large_n-13_eps-8_compute-2048k_lr-1e-3.pdf}&
\\[-2mm]
&
\includegraphics[height=1.\utilheightindhparamgptlargecompute]{fig/gpt2-large_n-13_eps-1_compute-4096k_lr-1e-3.pdf}&
\includegraphics[height=1.\utilheightindhparamgptlargecompute]{fig/gpt2-large_n-13_eps-2_compute-4096k_lr-1e-3.pdf}&
\includegraphics[height=1.\utilheightindhparamgptlargecompute]{fig/gpt2-large_n-13_eps-4_compute-4096k_lr-1e-3.pdf}&
\includegraphics[height=1.\utilheightindhparamgptlargecompute]{fig/gpt2-large_n-13_eps-8_compute-4096k_lr-1e-3.pdf}&
\\[-2mm]
\end{tabular}
}
\end{subfigure}
}
% \vspace{-2mm}
\caption{GPT2-large, fixed compute.}%
\label{fig:ind-hparam-gpt2-large-compute}
% \vspace{-1.2em}
\end{figure}



==> fig_desc/fig_individual_hparam_cmp_gpt2-large_iter.tex <==
\begin{figure}


% \captionsetup[subfigure]{labelformat=empty}

\newlength{\utilheightindhparamgptlargeiter}
\settoheight{\utilheightindhparamgptlargeiter}{\includegraphics[width=.3\columnwidth]{fig/gpt2-large_n-13_eps-1_b-2048_lr-1e-3.pdf}}%


\newcommand{\rowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\utilheightindhparamgptlargeiter][c]{\tiny #1}}}

\centering



{
\renewcommand{\tabcolsep}{10pt}



\begin{subfigure}[]{\columnwidth}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}c@{}}
        &  \makecell{\tiny{\textbf{}}}
        & \makecell{\tiny{\textbf{}}}
        &  \makecell{\tiny{\textbf{}}}
        % & \makecell{\tiny{\textbf{$p=1.0$, varying $T$}}}
        \\
&
\includegraphics[height=1.2\utilheightindhparamgptlargeiter]{fig/gpt2-large_n-13_eps-1_b-2048_lr-1e-3.pdf}&
\includegraphics[height=1.2\utilheightindhparamgptlargeiter]{fig/gpt2-large_n-13_eps-2_b-2048_lr-1e-3.pdf}&
\includegraphics[height=1.2\utilheightindhparamgptlargeiter]{fig/gpt2-large_n-13_eps-4_b-2048_lr-1e-3.pdf}&
\includegraphics[height=1.2\utilheightindhparamgptlargeiter]{fig/gpt2-large_n-13_eps-8_b-2048_lr-1e-3.pdf}&
\\[-2mm]
&
\includegraphics[height=1.2\utilheightindhparamgptlargeiter]{fig/gpt2-large_n-13_eps-1_b-4096_lr-1e-3.pdf}&
\includegraphics[height=1.2\utilheightindhparamgptlargeiter]{fig/gpt2-large_n-13_eps-2_b-4096_lr-1e-3.pdf}&
\includegraphics[height=1.2\utilheightindhparamgptlargeiter]{fig/gpt2-large_n-13_eps-4_b-4096_lr-1e-3.pdf}&
\includegraphics[height=1.2\utilheightindhparamgptlargeiter]{fig/gpt2-large_n-13_eps-8_b-4096_lr-1e-3.pdf}&
\\[-2mm]
&
\includegraphics[height=1.2\utilheightindhparamgptlargeiter]{fig/gpt2-large_n-13_eps-1_b-8192_lr-1e-3.pdf}&
\includegraphics[height=1.2\utilheightindhparamgptlargeiter]{fig/gpt2-large_n-13_eps-2_b-8192_lr-1e-3.pdf}&
\includegraphics[height=1.2\utilheightindhparamgptlargeiter]{fig/gpt2-large_n-13_eps-4_b-8192_lr-1e-3.pdf}&
\includegraphics[height=1.2\utilheightindhparamgptlargeiter]{fig/gpt2-large_n-13_eps-8_b-8192_lr-1e-3.pdf}&
\\[-2mm]
\end{tabular}}
\end{subfigure}
}
% \vspace{-2mm}
\caption{GPT2-large, varying iterations. }%
\label{fig:ind-hparam-gpt2-large-iter}
% \vspace{-1.2em}
\end{figure}



==> fig_desc/fig_individual_hparam_cmp_gpt2-large_lr.tex <==
\begin{figure}


% \captionsetup[subfigure]{labelformat=empty}

\newlength{\utilheightindhparamgptlargelr}
\settoheight{\utilheightindhparamgptlargelr}{\includegraphics[width=.3\columnwidth]{fig/gpt2-large_n-13_eps-1_b-2048_lr-1e-3.pdf}}%


\newcommand{\rowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\utilheightindhparamgptlargelr][c]{\tiny #1}}}

\centering



{
\renewcommand{\tabcolsep}{10pt}



\begin{subfigure}[]{\columnwidth}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}c@{}}
        &  \makecell{\tiny{\textbf{}}}
        & \makecell{\tiny{\textbf{}}}
        &  \makecell{\tiny{\textbf{}}}
        % & \makecell{\tiny{\textbf{$p=1.0$, varying $T$}}}
        \\
&
\includegraphics[height=1.\utilheightindhparamgptlargelr]{fig/gpt2-large_n-13_eps-1_b-4096_T-500.pdf}&
\includegraphics[height=1.\utilheightindhparamgptlargelr]{fig/gpt2-large_n-13_eps-2_b-4096_T-500.pdf}&
\includegraphics[height=1.\utilheightindhparamgptlargelr]{fig/gpt2-large_n-13_eps-4_b-4096_T-500.pdf}&
\includegraphics[height=1.\utilheightindhparamgptlargelr]{fig/gpt2-large_n-13_eps-8_b-4096_T-500.pdf}&
\\[-2mm]
\end{tabular}
}
\end{subfigure}
}
% \vspace{-2mm}
\caption{GPT2-large, varying learning rate}%
\label{fig:ind-hparam-gpt2-large-lr}
% \vspace{-1.2em}
\end{figure}



==> fig_desc/fig_individual_hparam_cmp_gpt2_bs.tex <==
\begin{figure}


% \captionsetup[subfigure]{labelformat=empty}

\newlength{\utilheightindhparamgptbs}
\settoheight{\utilheightindhparamgptbs}{\includegraphics[width=.3\columnwidth]{fig/gpt2-large_n-13_eps-1_b-2048_lr-1e-3.pdf}}%


\newcommand{\rowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\utilheightindhparamgptbs][c]{\tiny #1}}}

\centering



{
\renewcommand{\tabcolsep}{10pt}



\begin{subfigure}[]{\columnwidth}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}c@{}}
        &  \makecell{\tiny{\textbf{}}}
        & \makecell{\tiny{\textbf{}}}
        &  \makecell{\tiny{\textbf{}}}
        % & \makecell{\tiny{\textbf{$p=1.0$, varying $T$}}}
        \\
&
\includegraphics[height=1.\utilheightindhparamgptbs]{fig/gpt_n-14_eps-1_T-250_lr-3e-3.pdf}&
\includegraphics[height=1.\utilheightindhparamgptbs]{fig/gpt_n-14_eps-2_T-250_lr-3e-3.pdf}&
\includegraphics[height=1.\utilheightindhparamgptbs]{fig/gpt_n-14_eps-4_T-250_lr-3e-3.pdf}&
\includegraphics[height=1.\utilheightindhparamgptbs]{fig/gpt_n-14_eps-8_T-250_lr-3e-3.pdf}&
\\[-2mm]
&
\includegraphics[height=1.\utilheightindhparamgptbs]{fig/gpt_n-14_eps-1_T-500_lr-3e-3.pdf}&
\includegraphics[height=1.\utilheightindhparamgptbs]{fig/gpt_n-14_eps-2_T-500_lr-3e-3.pdf}&
\includegraphics[height=1.\utilheightindhparamgptbs]{fig/gpt_n-14_eps-4_T-500_lr-3e-3.pdf}&
\includegraphics[height=1.\utilheightindhparamgptbs]{fig/gpt_n-14_eps-8_T-500_lr-3e-3.pdf}&
\\[-2mm]
&
\includegraphics[height=1.\utilheightindhparamgptbs]{fig/gpt_n-14_eps-1_T-1000_lr-3e-3.pdf}&
\includegraphics[height=1.\utilheightindhparamgptbs]{fig/gpt_n-14_eps-2_T-1000_lr-3e-3.pdf}&
\includegraphics[height=1.\utilheightindhparamgptbs]{fig/gpt_n-14_eps-4_T-1000_lr-3e-3.pdf}&
\includegraphics[height=1.\utilheightindhparamgptbs]{fig/gpt_n-14_eps-8_T-1000_lr-3e-3.pdf}&
\\[-2mm]
\end{tabular}
}
\end{subfigure}
}
% \vspace{-2mm}
\caption{GPT2, varying batch size}%
\label{fig:ind-hparam-gpt2-bs}
% \vspace{-1.2em}
\end{figure}



==> fig_desc/fig_individual_hparam_cmp_gpt2_compute.tex <==
\begin{figure}


% \captionsetup[subfigure]{labelformat=empty}

\newlength{\utilheightindhparamgptcompute}
\settoheight{\utilheightindhparamgptcompute}{\includegraphics[width=.22\columnwidth]{fig/gpt2-large_n-13_eps-1_b-2048_lr-1e-3.pdf}}%

\newlength{\legendheightindhparamgptcompute}
\setlength{\legendheightindhparamgptcompute}{0.45\utilheightindhparamgptcompute}%




\newcommand{\rowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\utilheightindhparamgptcompute][c]{\tiny #1}}}

\centering



{
\renewcommand{\tabcolsep}{10pt}


\begin{subfigure}[]{\columnwidth}
\centering
\begin{tabular}{l}
\includegraphics[height=\legendheightindhparamgptcompute]{fig/legend_fix_compute_gpt2-large_cropped.pdf}
\end{tabular}
\end{subfigure}
\vspace{-1.5em}

\begin{subfigure}[]{\columnwidth}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}c@{}}
        &  \makecell{\tiny{\textbf{}}}
        & \makecell{\tiny{\textbf{}}}
        &  \makecell{\tiny{\textbf{}}}
        % & \makecell{\tiny{\textbf{$p=1.0$, varying $T$}}}
        \\
& 
\scriptsize{$\varepsilon=1$} &
\scriptsize{$\varepsilon=2$} &
\scriptsize{$\varepsilon=4$} &
\scriptsize{$\varepsilon=8$} &
\\
& 
\includegraphics[height=1.\utilheightindhparamgptcompute]{fig/gpt_n-14_eps-1_compute-1024k_lr-3e-3.pdf}&
\includegraphics[height=1.\utilheightindhparamgptcompute]{fig/gpt_n-14_eps-2_compute-1024k_lr-3e-3.pdf}&
\includegraphics[height=1.\utilheightindhparamgptcompute]{fig/gpt_n-14_eps-4_compute-1024k_lr-3e-3.pdf}&
\includegraphics[height=1.\utilheightindhparamgptcompute]{fig/gpt_n-14_eps-8_compute-1024k_lr-3e-3.pdf}&
\\[-2mm]
&
\includegraphics[height=1.\utilheightindhparamgptcompute]{fig/gpt_n-14_eps-1_compute-2048k_lr-3e-3.pdf}&
\includegraphics[height=1.\utilheightindhparamgptcompute]{fig/gpt_n-14_eps-2_compute-2048k_lr-3e-3.pdf}&
\includegraphics[height=1.\utilheightindhparamgptcompute]{fig/gpt_n-14_eps-4_compute-2048k_lr-3e-3.pdf}&
\includegraphics[height=1.\utilheightindhparamgptcompute]{fig/gpt_n-14_eps-8_compute-2048k_lr-3e-3.pdf}&
\\[-2mm]
\end{tabular}
}
\end{subfigure}
}
% \vspace{-2mm}
\caption{GPT2, fixed compute.}%
\label{fig:ind-hparam-gpt2-compute}
% \vspace{-1.2em}
\end{figure}



==> fig_desc/fig_individual_hparam_cmp_gpt2_iter.tex <==
\begin{figure}


% \captionsetup[subfigure]{labelformat=empty}

\newlength{\utilheightindhparamgptiter}
\settoheight{\utilheightindhparamgptiter}{\includegraphics[width=.3\columnwidth]{fig/gpt2-large_n-13_eps-1_b-2048_lr-1e-3.pdf}}%


\newcommand{\rowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\utilheightindhparamgptiter][c]{\tiny #1}}}

\centering



{
\renewcommand{\tabcolsep}{10pt}



\begin{subfigure}[]{\columnwidth}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}c@{}}
        &  \makecell{\tiny{\textbf{}}}
        & \makecell{\tiny{\textbf{}}}
        &  \makecell{\tiny{\textbf{}}}
        % & \makecell{\tiny{\textbf{$p=1.0$, varying $T$}}}
        \\
&
\includegraphics[height=1.2\utilheightindhparamgptiter]{fig/gpt_n-14_eps-1_b-1024_lr-3e-3.pdf}&
\includegraphics[height=1.2\utilheightindhparamgptiter]{fig/gpt_n-14_eps-2_b-1024_lr-3e-3.pdf}&
\includegraphics[height=1.2\utilheightindhparamgptiter]{fig/gpt_n-14_eps-4_b-1024_lr-3e-3.pdf}&
\includegraphics[height=1.2\utilheightindhparamgptiter]{fig/gpt_n-14_eps-8_b-1024_lr-3e-3.pdf}&
\\[-2mm]
&
\includegraphics[height=1.2\utilheightindhparamgptiter]{fig/gpt_n-14_eps-1_b-2048_lr-3e-3.pdf}&
\includegraphics[height=1.2\utilheightindhparamgptiter]{fig/gpt_n-14_eps-2_b-2048_lr-3e-3.pdf}&
\includegraphics[height=1.2\utilheightindhparamgptiter]{fig/gpt_n-14_eps-4_b-2048_lr-3e-3.pdf}&
\includegraphics[height=1.2\utilheightindhparamgptiter]{fig/gpt_n-14_eps-8_b-2048_lr-3e-3.pdf}&
\\[-2mm]
&
\includegraphics[height=1.2\utilheightindhparamgptiter]{fig/gpt_n-14_eps-1_b-4096_lr-3e-3.pdf}&
\includegraphics[height=1.2\utilheightindhparamgptiter]{fig/gpt_n-14_eps-2_b-4096_lr-3e-3.pdf}&
\includegraphics[height=1.2\utilheightindhparamgptiter]{fig/gpt_n-14_eps-4_b-4096_lr-3e-3.pdf}&
\includegraphics[height=1.2\utilheightindhparamgptiter]{fig/gpt_n-14_eps-8_b-4096_lr-3e-3.pdf}&
\\[-2mm]
&
\includegraphics[height=1.2\utilheightindhparamgptiter]{fig/gpt_n-14_eps-1_b-8192_lr-3e-3.pdf}&
\includegraphics[height=1.2\utilheightindhparamgptiter]{fig/gpt_n-14_eps-2_b-8192_lr-3e-3.pdf}&
\includegraphics[height=1.2\utilheightindhparamgptiter]{fig/gpt_n-14_eps-4_b-8192_lr-3e-3.pdf}&
\includegraphics[height=1.2\utilheightindhparamgptiter]{fig/gpt_n-14_eps-8_b-8192_lr-3e-3.pdf}&
\\[-2mm]
\end{tabular}}
\end{subfigure}
}
% \vspace{-2mm}
\caption{GPT2, varying iterations. TODO: 1. use one unified legend on top of the big figure, remove small legends in each subfigure; 2. consider changing the title format to e.g., (*, 4096, 1e-3); 3. consider adjusting the xlim and ylim manually---e.g., one fixed range for one epsilon value, to avoid inflated error bars, e.g., row 3 col 3}%
\label{fig:ind-hparam-gpt2-iter}
% \vspace{-1.2em}
\end{figure}



==> fig_desc/fig_individual_hparam_cmp_gpt2_lr.tex <==
\begin{figure}


% \captionsetup[subfigure]{labelformat=empty}

\newlength{\utilheightindhparamgptlr}
\settoheight{\utilheightindhparamgptlr}{\includegraphics[width=.3\columnwidth]{fig/gpt2-large_n-13_eps-1_b-2048_lr-1e-3.pdf}}%


\newcommand{\rowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\utilheightindhparamgptlr][c]{\tiny #1}}}

\centering



{
\renewcommand{\tabcolsep}{10pt}



\begin{subfigure}[]{\columnwidth}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}c@{}}
        &  \makecell{\tiny{\textbf{}}}
        & \makecell{\tiny{\textbf{}}}
        &  \makecell{\tiny{\textbf{}}}
        % & \makecell{\tiny{\textbf{$p=1.0$, varying $T$}}}
        \\
&
\includegraphics[height=1.\utilheightindhparamgptlr]{fig/gpt_n-14_eps-1_b-8192_T-250.pdf}&
\includegraphics[height=1.\utilheightindhparamgptlr]{fig/gpt_n-14_eps-2_b-8192_T-250.pdf}&
\includegraphics[height=1.\utilheightindhparamgptlr]{fig/gpt_n-14_eps-4_b-8192_T-250.pdf}&
\includegraphics[height=1.\utilheightindhparamgptlr]{fig/gpt_n-14_eps-8_b-8192_T-250.pdf}&
\\[-2mm]
\end{tabular}
}
\end{subfigure}
}
% \vspace{-2mm}
\caption{GPT2, varying learning rate}%
\label{fig:ind-hparam-gpt2-lr}
% \vspace{-1.2em}
\end{figure}



==> fig_desc/fig_profile_accountants_vary_eps_archive.tex <==
\begin{figure*}[!h]


% \captionsetup[subfigure]{labelformat=empty}

\newlength{\utilheightprofacctvaryeps}
\settoheight{\utilheightprofacctvaryeps}{\includegraphics[width=.33\linewidth]{fig/acr_var_gpt2.pdf}}%


\newlength{\legendheightprofacctvaryeps}
\setlength{\legendheightprofacctvaryeps}{0.14\utilheightprofacctvaryeps}%


\newcommand{\rowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\utilheightprofacctvaryeps][c]{\tiny #1}}}

\centering



{
\renewcommand{\tabcolsep}{10pt}


% \begin{subfigure}[]{\linewidth}
% \centering
% \begin{tabular}{l}
% \includegraphics[height=\legendheightprofacctvaryeps]{fig/legend_tofu_all_subgroups.pdf}
% \end{tabular}
% \end{subfigure}

% \vspace{-1em}

\begin{subfigure}[]{\linewidth}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}c@{}}
        & \makecell[c]{\quad\small \textbf{(a)} RDP accountant}
        &  \makecell[c]{\quad\small \textbf{(b)} PRV accountant}
        &  \makecell[c]{\quad\qquad\small \textbf{(c)} Connect-the-Dots accountant}
        % &  \makecell{\small{{(d)}}}
        \\[-1mm]
\rowname{\normalsize{\qquad \bm{$\eps=1$}}}
&
\includegraphics[height=\utilheightprofacctvaryeps]{fig/fig_privacy_profile_rdp_eps-1-1e-06_s1.pdf}
&
\includegraphics[height=\utilheightprofacctvaryeps]{fig/fig_privacy_profile_prv_eps-1-1e-06_s1.pdf}
&
\includegraphics[height=\utilheightprofacctvaryeps]{fig/fig_privacy_profile_cd_eps-1-1e-06_s1.pdf}
\\[-1mm]
\rowname{\normalsize{\qquad \bm{$\eps=2$}}}
&
\includegraphics[height=\utilheightprofacctvaryeps]{fig/fig_privacy_profile_rdp_eps-2-1e-06_s1.pdf}
&
\includegraphics[height=\utilheightprofacctvaryeps]{fig/fig_privacy_profile_prv_eps-2-1e-06_s1.pdf}
&
\includegraphics[height=\utilheightprofacctvaryeps]{fig/fig_privacy_profile_cd_eps-2-1e-06_s1.pdf}
\\[-1mm]
\rowname{\normalsize{\qquad \bm{$\eps=4$}}}
&
\includegraphics[height=\utilheightprofacctvaryeps]{fig/fig_privacy_profile_rdp.pdf}
&
\includegraphics[height=\utilheightprofacctvaryeps]{fig/fig_privacy_profile.pdf}
&
\includegraphics[height=\utilheightprofacctvaryeps]{fig/fig_privacy_profile_connect_dots.pdf}
\\[-1mm]
\rowname{\normalsize{\qquad \bm{$\eps=8$}}}
&
\includegraphics[height=\utilheightprofacctvaryeps]{fig/fig_privacy_profile_rdp_eps-8-1e-06_s1.pdf}
&
\includegraphics[height=\utilheightprofacctvaryeps]{fig/fig_privacy_profile_prv_eps-8-1e-06_s1.pdf}
&
\includegraphics[height=\utilheightprofacctvaryeps]{fig/fig_privacy_profile_cd_eps-8-1e-06_s1.pdf}
\\[-3mm]
\end{tabular}}
\end{subfigure}
}
% \vspace{-2mm}
\caption{\textbf{Privacy profiles for different target \bm{$\eps\in \{1,2,4,8\}$} (reflected in rows)}  under different accountants (reflected in columns): $n=180,000$, $b=4096$,
target=$(\eps, 10^{-6})$-DP.
}%
\label{fig:profile-accountants-vary-eps}
\end{figure*}



==> fig_desc/fig_result_1_gpt2.tex <==
\begin{figure}


% \captionsetup[subfigure]{labelformat=empty}

\newlength{\utilheightgoodreadschatcmp}
\settoheight{\utilheightgoodreadschatcmp}{\includegraphics[width=.5\columnwidth]{fig/acr_var_gpt2.pdf}}%


\newlength{\legendheightgoodreadschatcmp}
\setlength{\legendheightgoodreadschatcmp}{0.23\utilheightgoodreadschatcmp}%


\newcommand{\rowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\utilheightgoodreadschatcmp][c]{\tiny #1}}}

\centering



{
\renewcommand{\tabcolsep}{10pt}


% \begin{subfigure}[]{\columnwidth}
% \begin{tabular}{l}
% \includegraphics[height=\legendheightgoodreadschatcmp]{figs/legend_fade.png}\\[-2mm]
% \includegraphics[height=.6\legendheightgoodreadschatcmp]{figs/fig_legend_chat_cmp.png}
% \end{tabular}
% \end{subfigure}

% \vspace{-1em}

\begin{subfigure}[]{\columnwidth}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}c@{}c@{}c@{}}
        & \makecell{\small{{GPT2}}}
        &  \makecell{\small{{GPT2-Large}}}
        \\[-1mm]
\rowname{\small{ACR}}&
\includegraphics[height=\utilheightgoodreadschatcmp]{fig/acr_var_gpt2_dp.pdf}&
\includegraphics[height=\utilheightgoodreadschatcmp]{fig/acr_var_gpt2-large_dp.pdf}
\\
\rowname{\small{Exact Match Ratio}}&\includegraphics[height=\utilheightgoodreadschatcmp]{fig/emr_var_gpt2_dp.pdf}&
\includegraphics[height=\utilheightgoodreadschatcmp]{fig/emr_var_gpt2-large_dp.pdf}
\\[-3mm]
&\small{$\varepsilon$}&\small{$\varepsilon$}\\
\end{tabular}}
\end{subfigure}
}
% \vspace{-2mm}
\caption{caption
}%
\label{fig:1}
% \vspace{-1.2em}
\end{figure}



==> fig_desc/fig_sel_quality_full.tex <==
\begin{figure}


% \captionsetup[subfigure]{labelformat=empty}

\newlength{\utilheightselqualityfull}
\settoheight{\utilheightselqualityfull}{\includegraphics[width=.5\linewidth]{fig/acr_var_gpt2.pdf}}%


\newlength{\legendheightselqualityfull}
% \setlength{\legendheightselqualityfull}{0.06\utilheightselqualityfull}%
\settoheight{\legendheightselqualityfull}{\includegraphics[width=\linewidth]{fig/legend_rel_error_cropped.pdf}}%



\newcommand{\rowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\utilheightselqualityfull][c]{\tiny #1}}}

\centering



{
\renewcommand{\tabcolsep}{10pt}


\begin{subfigure}[]{\linewidth}
\centering
\begin{tabular}{l}
\includegraphics[height=.4\legendheightselqualityfull]{fig/legend_rel_error_cropped.pdf}\\
\end{tabular}
\end{subfigure}

\vspace{1mm}

\begin{subfigure}[]{.6\linewidth}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}c@{}}
        & \makecell[c]{\Large \qquad\textbf{(a)} GPT-2-S on Enron}
        &  \makecell[c]{\Large \qquad\qquad\textbf{(b)} GPT-2-L on Enron}
        % &  \makecell[c]{\small \textbf{(c)} Llama-2-7b on density-adjusted TOFU \\ \small \textbf{Dimension: dataset} (increased secret density)}
        % &  \makecell{\small{{(d)}}}
        \\[-1mm]
% \rowname{\small{ACR}}
&
\includegraphics[height=\utilheightselqualityfull]{fig/suboptimality_ratio_resample_mean_gpt2_criteria-earlier-ftr1_cmp_all.pdf}
&
\includegraphics[height=\utilheightselqualityfull]{fig/suboptimality_ratio_resample_mean_gpt2-large_criteria-earlier-ftr1_cmp_all.pdf}
% &
% \includegraphics[height=\utilheightselqualityfull]{fig/var_measures.pdf}
\\[-3mm]
\end{tabular}}
\end{subfigure}


\begin{subfigure}[]{.9\linewidth}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}c@{}}
        & \makecell[c]{\Large\qquad \textbf{(c)} Llama-2-7b on TOFU-1}
        &  \makecell[c]{\Large\qquad \textbf{(d)} Llama-2-7b on TOFU-2}
        &  \makecell[c]{\Large\qquad \textbf{(e)} Llama-2-7b on TOFU-4}
        % &  \makecell[c]{\small \textbf{(c)} Llama-2-7b on density-adjusted TOFU \\ \small \textbf{Dimension: dataset} (increased secret density)}
        % &  \makecell{\small{{(d)}}}
        \\
% \rowname{\small{ACR}}
&
\includegraphics[height=\utilheightselqualityfull]{fig/suboptimality_ratio_resample_mean_tofu-1_criteria-earlier-ftr1_cmp_all.pdf}
&
\includegraphics[height=\utilheightselqualityfull]{fig/suboptimality_ratio_resample_mean_tofu-2_criteria-earlier-ftr1_cmp_all.pdf}
&
\includegraphics[height=\utilheightselqualityfull]{fig/suboptimality_ratio_resample_mean_tofu-4_criteria-earlier-ftr1_cmp_all.pdf}
% &
% \includegraphics[height=\utilheightselqualityfull]{fig/var_measures.pdf}
\\[-3mm]
\end{tabular}}
\end{subfigure}

}
% \vspace{-2mm}
\caption{Relative privacy risk of our procedure compared with baselines in all settings corresponding to different models and datasets, across varying $\eps$'s.}%
\label{fig:relative-error-full}
% \vspace{-1.2em}
\end{figure}


==> fig_desc/fig_selection_gpt2-large.tex <==
\begin{figure*}


% \captionsetup[subfigure]{labelformat=empty}

\newlength{\utilheightselectiongptlargeepsc}
\settoheight{\utilheightselectiongptlargeepsc}{\includegraphics[width=.22\linewidth]{fig/gpt2-large_n-13_eps-1_b-2048_lr-1e-3.pdf}}%


\newcommand{\rowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\utilheightselectiongptlargeepsc][c]{\tiny #1}}}

\centering



{
\renewcommand{\tabcolsep}{10pt}



\begin{subfigure}[]{\linewidth}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}c@{}}
        &  \makecell{\tiny{\textbf{}}}
        & \makecell{\tiny{\textbf{}}}
        &  \makecell{\tiny{\textbf{}}}
        % & \makecell{\tiny{\textbf{$p=1.0$, varying $T$}}}
        \\
\rowname{$\varepsilon=1$}&
\includegraphics[height=1.\utilheightselectiongptlargeepsc]{fig/stepwise_gpt2-large_n-13_eps-1_step-0.pdf}&
\includegraphics[height=1.\utilheightselectiongptlargeepsc]{fig/stepwise_gpt2-large_n-13_eps-1_step-1.pdf}&
\includegraphics[height=1.\utilheightselectiongptlargeepsc]{fig/stepwise_gpt2-large_n-13_eps-1_step-2.pdf}&
\includegraphics[height=1.\utilheightselectiongptlargeepsc]{fig/stepwise_gpt2-large_n-13_eps-1_step-3.pdf}&
\\[-2mm]
\rowname{$\varepsilon=2$}&
\includegraphics[height=1.\utilheightselectiongptlargeepsc]{fig/stepwise_gpt2-large_n-13_eps-2_step-0.pdf}&
\includegraphics[height=1.\utilheightselectiongptlargeepsc]{fig/stepwise_gpt2-large_n-13_eps-2_step-1.pdf}&
\includegraphics[height=1.\utilheightselectiongptlargeepsc]{fig/stepwise_gpt2-large_n-13_eps-2_step-2.pdf}&
\includegraphics[height=1.\utilheightselectiongptlargeepsc]{fig/stepwise_gpt2-large_n-13_eps-2_step-3.pdf}&
\\[-2mm]
\rowname{$\varepsilon=4$}&
\includegraphics[height=1.\utilheightselectiongptlargeepsc]{fig/stepwise_gpt2-large_n-13_eps-4_step-0.pdf}&
\includegraphics[height=1.\utilheightselectiongptlargeepsc]{fig/stepwise_gpt2-large_n-13_eps-4_step-1.pdf}&
\includegraphics[height=1.\utilheightselectiongptlargeepsc]{fig/stepwise_gpt2-large_n-13_eps-4_step-2.pdf}&
\includegraphics[height=1.\utilheightselectiongptlargeepsc]{fig/stepwise_gpt2-large_n-13_eps-4_step-3.pdf}&
\\[-2mm]
\rowname{$\varepsilon=8$}&
\includegraphics[height=1.\utilheightselectiongptlargeepsc]{fig/stepwise_gpt2-large_n-13_eps-8_step-0.pdf}&
\includegraphics[height=1.\utilheightselectiongptlargeepsc]{fig/stepwise_gpt2-large_n-13_eps-8_step-1.pdf}&
\includegraphics[height=1.\utilheightselectiongptlargeepsc]{fig/stepwise_gpt2-large_n-13_eps-8_step-2.pdf}&
\includegraphics[height=1.\utilheightselectiongptlargeepsc]{fig/stepwise_gpt2-large_n-13_eps-8_step-3.pdf}&
\\[-2mm]
\end{tabular}
}
\end{subfigure}
}
% \vspace{-2mm}
\caption{GPT2-large.}%
\label{fig:select-gpt2-large}
% \vspace{-1.2em}
\end{figure*}



==> fig_desc/fig_selection_gpt2.tex <==
\begin{figure*}


% \captionsetup[subfigure]{labelformat=empty}

\newlength{\utilheightselectiongptepsc}
\settoheight{\utilheightselectiongptepsc}{\includegraphics[width=.22\linewidth]{fig/gpt2-large_n-13_eps-1_b-2048_lr-1e-3.pdf}}%


\newlength{\legendheightindselectiongpt}
\setlength{\legendheightindselectiongpt}{0.45\utilheightselectiongptepsc}%



\newcommand{\rowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\utilheightselectiongptepsc][c]{\tiny #1}}}

\centering



{
\renewcommand{\tabcolsep}{10pt}



\begin{subfigure}[]{\textwidth}
\centering
\begin{tabular}{l}
\includegraphics[height=.28\legendheightindselectiongpt]{fig/color_legend_cropped.pdf}\\
\includegraphics[height=.28\legendheightindselectiongpt]{fig/marker_legend_cropped.pdf}\\
\end{tabular}
\end{subfigure}
\vspace{-1.5em}


\begin{subfigure}[]{\linewidth}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}c@{}}
        &  \makecell{\tiny{\textbf{}}}
        & \makecell{\tiny{\textbf{}}}
        &  \makecell{\tiny{\textbf{}}}
        % & \makecell{\tiny{\textbf{$p=1.0$, varying $T$}}}
        \\
\rowname{$\varepsilon=8$}&
\includegraphics[height=1.\utilheightselectiongptepsc]{fig/stepwise_gpt2_n-14_eps-8_step-0.pdf}&
\includegraphics[height=1.\utilheightselectiongptepsc]{fig/stepwise_gpt2_n-14_eps-8_step-1.pdf}&
\includegraphics[height=1.\utilheightselectiongptepsc]{fig/stepwise_gpt2_n-14_eps-8_step-2.pdf}&
\includegraphics[height=1.\utilheightselectiongptepsc]{fig/stepwise_gpt2_n-14_eps-8_step-3.pdf}&
\\[-2mm]
\end{tabular}
}
\end{subfigure}
}
% \vspace{-2mm}
\caption{GPT2. black bounding box: retained datapoints; hatch pattern: best datapoint. 
TODO: compare with baseline: 1) a random point on the left; 2) the highest loss point on the left;
TODO: also report the number of datapoints retained (hopefully no more than 3); if more than 1, choose a random one?}%
\label{fig:select-gpt2}
% \vspace{-1.2em}
\end{figure*}



==> fig_desc/fig_selection_llama.tex <==
\begin{figure*}


% \captionsetup[subfigure]{labelformat=empty}

\newlength{\utilheightselectionllamaepsc}
\settoheight{\utilheightselectionllamaepsc}{\includegraphics[width=.22\linewidth]{fig/gpt2-large_n-13_eps-1_b-2048_lr-1e-3.pdf}}%


\newlength{\legendheightindselectionllama}
\setlength{\legendheightindselectionllama}{0.45\utilheightselectionllamaepsc}%



\newcommand{\rowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\utilheightselectionllamaepsc][c]{\tiny #1}}}

\centering



{
\renewcommand{\tabcolsep}{10pt}



% \begin{subfigure}[]{\textwidth}
% \centering
% \begin{tabular}{l}
% \includegraphics[height=.28\legendheightindselectionllama]{fig/color_legend_cropped.pdf}\\
% \includegraphics[height=.28\legendheightindselectionllama]{fig/marker_legend_cropped.pdf}\\
% \end{tabular}
% \end{subfigure}
% \vspace{-1.5em}


\begin{subfigure}[]{\linewidth}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}c@{}}
        &  \makecell{\tiny{\textbf{}}}
        & \makecell{\tiny{\textbf{}}}
        &  \makecell{\tiny{\textbf{}}}
        % & \makecell{\tiny{\textbf{$p=1.0$, varying $T$}}}
        \\
% \rowname{$\varepsilon=2$}
&
\includegraphics[height=1.\utilheightselectionllamaepsc]{fig/stepwise_llama_eps-2_step-0.pdf}& 
\includegraphics[height=1.\utilheightselectionllamaepsc]{fig/stepwise_llama_eps-2_step-1.pdf}&
\includegraphics[height=1.\utilheightselectionllamaepsc]{fig/stepwise_llama_eps-2_step-2.pdf}&
% \includegraphics[height=1.\utilheightselectionllamaepsc]{fig/stepwise_llama_eps-2_step-3.pdf}&
\\[-2mm]
\end{tabular}
}
\end{subfigure}
}
% \vspace{-2mm}
\caption{llama2.}%
\label{fig:select-llama}
% \vspace{-1.2em}
\end{figure*}



==> fig_desc/tab_corr_subsets.tex <==
\begin{figure*}[!h]


% \captionsetup[subfigure]{labelformat=empty}

\newlength{\utilheightcorrsubset}
\settoheight{\utilheightcorrsubset}{\includegraphics[width=.33\linewidth]{fig/acr_var_gpt2.pdf}}%


\newlength{\legendheightcorrsubset}
\setlength{\legendheightcorrsubset}{0.14\utilheightcorrsubset}%


\newcommand{\rowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\utilheightcorrsubset][c]{\tiny #1}}}

\centering



{
\renewcommand{\tabcolsep}{10pt}


\begin{subfigure}[]{\linewidth}
\centering
\begin{tabular}{l}
\includegraphics[height=\legendheightcorrsubset]{fig/legend_gpt2_vs_gpt2l.pdf}
\end{tabular}
\end{subfigure}

% \vspace{-1em}

\begin{subfigure}[]{.67\linewidth}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}c@{}}
% \rowname{\normalsize{\qquad\textbf{ACR}}}
&
\includegraphics[height=1.05\utilheightcorrsubset]{fig/var_acr_gpt2s_eps-1-2-4-8_agg_upd.pdf}
&
\includegraphics[height=1.05\utilheightcorrsubset]{fig/var_acr_gpt2l_eps-1-2-4-8_agg_upd.pdf}
\\[-1mm]
% \rowname{\normalsize{\qquad\textbf{VMR}}}
&
\includegraphics[height=\utilheightcorrsubset]{fig/var_vmr_gpt2s_eps-1-2-4-8_agg.pdf}
&
\includegraphics[height=\utilheightcorrsubset]{fig/var_vmr_gpt2l_eps-1-2-4-8_agg.pdf}
\\[-1mm]
\end{tabular}}
\end{subfigure}
}
% \vspace{-2mm}
\caption{
\textbf{Empirical privacy variance across different \empv measures (ACR and VMR).}
\textit{Rows} correspond to different \empv measures:
(top) ACR; (bottom) VMR.
Columns correspond to different model sizes:
(left) GPT-2-S; (right) GPT-2-L.
Each subfigure shows \empv scores achieved by models trained using different configuration at different $\varepsilon$'s.
Each group's standard deviation is labeled at the top of its cluster.
The results show that, for both empirical privacy measures, \empvv increases as either $\varepsilon$ or model size grows.
% \textcolor{red}{TODO: add two points for GPT-2-L ACR figure (upper right)}
}%
\label{fig:var-enron-measure}
% \vspace{-1.2em}
\end{figure*}


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

